Comparison of Minimization Methods for Rosenbrock Functions

This paper gives an in-depth review of the most common iterative methods for unconstrained optimization using two functions that belong to a class of Rosenbrock functions as a performance test. This study covers the Steepest Gradient Descent Method, the Newton-Raphson Method, and the Fletcher-Reeves Conjugate Gradient method. In addition, four different step-size selecting methods including fixed-step-size, variable step-size, quadratic-fit, and golden section method were considered. Due to the computational nature of solving minimization problems, testing the algorithms is an essential part of this paper. Therefore, an extensive set of numerical test results is also provided to present an insightful and a comprehensive comparison of the reviewed algorithms. This study highlights the differences and the trade-offs involved in comparing these algorithms.

==> commented_out.tex <==
\begin{comment}
The table and simulations that summarize convergence for different types of optimization methods considered are indicated below:
\begin{figure*}\label{Table1}
 \caption{Table for the Steepest Descent}
    \centering
    \includegraphics[width=17cm]{firstorder.PNG}
    \label{fig:iteration1}
\end{figure*}

\begin{figure*}\label{Table2}
 \caption{Table for Newton and Conjugate Gradient}
    \centering
    \includegraphics[width=17cm]{secondorder.PNG}
    \label{fig:iteration1}
\end{figure*}
\end{comment}

\begin{comment}
\begin{figure}[h]
 \caption{Simulations for Steepest descent with fixed step size for function \ref{regularagentminimization} with initial $(2,2)$}
    \centering
    \includegraphics[width=4cm]{steepestfixed22first.PNG}
    \label{fig:iteration1}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Steepest descent with fixed step size for function \ref{regularagentminimization} with initial $(5,5)$}
    \centering
    \includegraphics[width=4cm]{steepestfixed55first.PNG}
    \label{fig:iteration2}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Steepest descent with fixed step size for function \ref{maliciousagentminimization} with initial $(2,2)$}
    \centering
    \includegraphics[width=4cm]{steepestfixed22second.PNG}
    \label{fig:iteration3}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Steepest descent with fixed step size for function \ref{maliciousagentminimization} with initial $(5,5)$}
    \centering
    \includegraphics[width=4cm]{steepestfixed22second.PNG}
    \label{fig:iteration4}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Steepest descent with variable step size for function \ref{regularagentminimization} with initial $(2,2)$}
    \centering
    \includegraphics[width=4cm]{variable22first.PNG}
    \label{fig:iteration5}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Steepest descent with variable step size for function \ref{regularagentminimization} with initial $(5,5)$}
    \centering
    \includegraphics[width=4cm]{variable55first.PNG}
    \label{fig:iteration6}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Steepest descent with variable step size for function \ref{maliciousagentminimization} with initial $(2,2)$}
    \centering
    \includegraphics[width=4cm]{variable22second.PNG}
    \label{fig:iteration7}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Steepest descent with variable step size for function \ref{maliciousagentminimization} with initial $(5,5)$}
    \centering
    \includegraphics[width=4cm]{variable55second.PNG}
    \label{fig:iteration8}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Steepest descent with quadratic fit for function \ref{regularagentminimization} with initial $(2,2)$}
    \centering
    \includegraphics[width=4cm]{quadratic22first.PNG}
    \label{fig:iteration9}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Steepest descent with quadratic fit for function \ref{regularagentminimization} with initial $(5,5)$}
    \centering
    \includegraphics[width=4cm]{quadratic55first.PNG}
    \label{fig:iteration10}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Steepest descent with quadratic fit for function \ref{maliciousagentminimization} with initial $(2,2)$}
    \centering
    \includegraphics[width=4cm]{quadratic22second.PNG}
    \label{fig:iteration11}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Steepest descent with quadratic fit for function \ref{maliciousagentminimization} with initial $(5,5)$}
    \centering
    \includegraphics[width=4cm]{quadratic55second.PNG}
    \label{fig:iteration12}
    \end{figure}
    \begin{figure}[h]
 \caption{Simulations for Steepest descent with golden section for function \ref{regularagentminimization} with initial $(2,2)$}
    \centering
    \includegraphics[width=4cm]{golden22first.PNG}
    \label{fig:iteration13}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Steepest descent with golden section for function \ref{regularagentminimization} with initial $(5,5)$}
    \centering
    \includegraphics[width=4cm]{golden55first.PNG}
    \label{fig:iteration14}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Steepest descent with golden section for function \ref{maliciousagentminimization} with initial $(2,2)$}
    \centering
    \includegraphics[width=4cm]{golden22second.PNG}
    \label{fig:iteration15}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Steepest descent with golden section for function \ref{maliciousagentminimization} with initial $(5,5)$}
    \centering
    \includegraphics[width=4cm]{golden55second.PNG}
    \label{fig:iteration16}
    \end{figure}
    \begin{figure}[h]
 \caption{Simulations for Newton method for function \ref{regularagentminimization} with initial $(2,2)$}
    \centering
    \includegraphics[width=4cm]{newton22first.PNG}
    \label{fig:iteration17}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Newton method for function \ref{regularagentminimization} with initial $(5,5)$}
    \centering
    \includegraphics[width=4cm]{newton55first.PNG}
    \label{fig:iteration18}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Newton method for function \ref{maliciousagentminimization} with initial $(2,2)$}
    \centering
    \includegraphics[width=4cm]{newton22second.PNG}
    \label{fig:iteration19}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Newton method for function \ref{maliciousagentminimization} with initial $(5,5)$}
    \centering
    \includegraphics[width=4cm]{newton55second.PNG}
    \label{fig:iteration20}
    \end{figure}
     \begin{figure}[h]
 \caption{Simulations for Conjugate gradient for function \ref{regularagentminimization} with initial $(2,2)$}
    \centering
    \includegraphics[width=4cm]{conjugate22first.PNG}
    \label{fig:iteration21}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Conjugate gradient for function \ref{regularagentminimization} with initial $(5,5)$}
    \centering
    \includegraphics[width=4cm]{conjugate55first.PNG}
    \label{fig:iteration22}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Conjugate gradient for function \ref{maliciousagentminimization} with initial $(2,2)$}
    \centering
    \includegraphics[width=4cm]{conjugate22second.PNG}
    \label{fig:iteration23}
\end{figure}
\begin{figure}[h]
 \caption{Simulations for Conjugate gradient for function \ref{maliciousagentminimization} with initial $(5,5)$}
    \centering
    \includegraphics[width=4cm]{conjugate55second.PNG}
    \label{fig:iteration24}
    \end{figure}
    \end{comment}
    
\begin{comment}
\begin{tabularx}{0.8\textwidth} { 
  | >{\raggedright\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\raggedleft\arraybackslash}X | }
 \hline
 item 11 & item 12 & item 13 \\
 \hline
 item 21  & item 22  & item 23  \\
\hline
item 31  & item 32  & item 33  \\
\hline
item 41  & item 42  & item 43 \\
\hline
\end{tabularx}
\end{comment}
